Relaxing Accurate Initialization Constraint for 3D Gaussian Splatting

3D Gaussian splatting (3DGS) has recently demonstrated impressive capabilities in real-time novel view synthesis and 3D reconstruction. However, 3DGS heavily depends on the accurate initialization derived from Structure-from-Motion (SfM) methods. When the quality of the initial point cloud deteriorates, such as in the presence of noise or when using randomly initialized point cloud, 3DGS often undergoes large performance drops. To address this limitation, we propose a novel optimization strategy dubbed RAIN-GS (Relaing Accurate Initialization Constraint for 3D Gaussian Splatting). Our approach is based on an in-depth analysis of the original 3DGS optimization scheme and the analysis of the SfM initialization in the frequency domain. Leveraging simple modifications based on our analyses, RAIN-GS successfully trains 3D Gaussians from sub-optimal point cloud (e.g., randomly initialized point cloud), effectively relaxing the need for accurate initialization. We demonstrate the efficacy of our strategy through quantitative and qualitative comparisons on multiple datasets, where RAIN-GS trained with random point cloud achieves performance on-par with or even better than 3DGS trained with accurate SfM point cloud. Our project page and code can be found at https://ku-cvlab.github.io/RAIN-GS.

==> assets/table/mip360_noisesfm_quan.tex <==
\begin {table*}[t]
    \caption{\textbf{Quantitative comparison on Mip-NeRF360 dataset in noisy SfM points setting}. We compare our method with 3DGS in noisy SfM points setting, We report PSNR, SSIM and LPIPS and color each cell as \colorbox{yzybest}{best}, \colorbox{yzysecond}{second best} and \colorbox{yzythird}{third best}.
    }
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|ccc|ccc|ccc|ccc|ccc}
        \hline \multirow[c]{3}{*}{ Method } & \multirow[c]{3}{*}{ \shortstack{Noisy \\ points}} & \multicolumn{15}{c}{Outdoor Scene} \\
        \cline{3-17}
         & & \multicolumn{3}{c|}{ bicycle } & \multicolumn{3}{c|}{ flowers } & \multicolumn{3}{c|}{ garden } & \multicolumn{3}{c|}{ stump } & \multicolumn{3}{c}{ treehill }\\
        & & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ &PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$  \\
        \hline

        3DGS & full  & 24.289& 0.692& 0.307& 21.028& 0.565& 0.374& 26.515& 0.846&0.133& 26.028& 0.743& 0.252& 21.728& 0.607& 0.380\\
        \hline
        
        Ours & cluster  & \third{24.598} & \third{0.706}& \third{0.281}& \second{21.761}& \third{0.614}&\second{0.325}& \third{26.679}& \third{0.850}& \third{0.116}& \third{26.555}& \third{0.764}& \third{0.219}& \third{22.379}& \second{0.625}& \best{0.334}\\

        Ours & <10\%  & \best{25.046}& \best{0.747}& \best{0.237}&  \third{21.748}& \best{0.618}& \third{0.327}& \best{26.932}& \best{0.855}& \second{0.115}& \best{26.686}& \best{0.772}& \best{0.213}& \second{22.486}& \best{0.630}& \second{0.335}\\
        
        Ours &\ding{55}  & \second 25.042& \best 0.747& \second 0.238&  \best 21.762& \second 0.616& \best 0.324&  \second 26.884& \second 0.854& \best 0.114& \second 26.680& \second 0.768& \second 0.215&  \best 22.528& \third 0.621& \third 0.342\\

        \hline
        \multicolumn{17}{c}{}
        \\
        \hline
        \multirow[c]{3}{*}{ Method } & \multirow[c]{3}{*}{ \shortstack{Noisy \\ points}} & \multicolumn{15}{c}{Indoor Scene} \\
        \cline{3-17} & & \multicolumn{3}{c|}{ room } & \multicolumn{3}{c|}{ counter } & \multicolumn{3}{c|}{ kitchen} & \multicolumn{3}{c|}{ bonsai } & \multicolumn{3}{c}{ average } \\
        
        & & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$  \\
        \hline

        3DGS  & full  &\second{30.740}& 0.901& 0.260& 23.872& 0.838& 0.285& 24.477& 0.877& 0.175& \third{25.823}&\third{0.875}& \third{0.265}& 24.944& 0.771& 0.270\\
        \hline

        Ours & cluster  & \third{30.698}& \best{0.906}& \third{0.249}& \second{28.305}& \second{0.893}& \best{0.220}&\second{ 31.055}& \best{0.920}&\best 0.136& \second{31.523}& \second{0.934}& \second{0.218}& \second{27.061}& \second{0.801}& \second{0.233}\\

        Ours & <10\% & 30.352& \second{0.904}& \second{0.248}& 
        \third{27.125}& \third{0.880}& \third{0.229}& \third{29.299}& \third{0.909}& \third{0.146}&  22.037& 0.781& 0.333&  \third{25.746}& \third{0.788}& \third{0.243}\\

        Ours & \ding{55}  & \best 30.809& \best 0.906& \best 0.247& \best 28.529& \best 0.895& \second 0.223& \best 31.270& \best 0.920& \second 0.137&  \best 31.547& \best 0.934& \best 0.218&  \best 27.228& \best 0.807& \best 0.229\\

        \hline
    \end{tabular}}

    \label{tab:noise_mip360}
\end{table*}


==> assets/table/mip360_sfm_quan.tex <==
\begin {table*}[t]
    \caption{\textbf{Quantitative comparison on Mip-NeRF360 dataset in sparse SfM points setting}. We compare our method with 3DGS in sparse SfM points setting, We report PSNR, SSIM and LPIPS and color each cell as \colorbox{yzybest}{best}, \colorbox{yzysecond}{second best} and \colorbox{yzythird}{third best}.
    }
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|ccc|ccc|ccc|ccc|ccc}
        \hline \multirow[c]{3}{*}{ Method } & \multirow[c]{3}{*}{ \shortstack{SfM \\ points}} & \multicolumn{15}{c}{Outdoor Scene} \\
        \cline{3-17}
         & & \multicolumn{3}{c|}{ bicycle } & \multicolumn{3}{c|}{ flowers } & \multicolumn{3}{c|}{ garden } & \multicolumn{3}{c|}{ stump } & \multicolumn{3}{c}{ treehill }\\
        & & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ &PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$  \\
        \hline

        3DGS & cluster  & 24.432& 0.699& 0.288& 20.959& 0.554& 0.379& 26.484& 0.842&0.127& 25.484& 0.718& 0.266& 21.704& 0.586& 0.391\\

        3DGS & <10\%  & 24.456& 0.700& 0.294& 21.260& 0.580& 0.360& 26.832& 0.850&0.127& 26.165& 0.744& 0.247& 22.260& 0.612& 0.365\\

        3DGS & full  & \best{25.246}& \best{0.771} & \best{ 0.205}& \third 21.520& \third \third 0.605& \third 0.336& \best{27.410}& \best{0.868}&\best{ 0.103}& \third 26.550& \second{0.775}& \third {0.210}& \third 22.490& \best{0.638}& \best{0.317}\\
        \hline
        
        Ours & cluster  & \third 25.100& \third 0.756& \third 0.224 & \second{21.744}& \second{0.616}&\second{0.321}& \third {27.016}& \third {0.859}& \second{0.106}& \second{26.692}& \third {0.772}& \second {0.208}& \second{22.496}& \third 0.629& \third 0.331\\

        Ours & <10\%  & \second{25.214} & \second{0.769} & \second{0.208} &  \best{21.858}& \best{0.619}& \best{0.320}& \second{27.130} & \second{0.861} & \third 0.107& \best{26.899}& \best{0.777}& \best{0.202}& \best{22.618}& \second{0.632} & \second{0.327} \\

        % \Xhline{3\arrayrulewidth}
        \hline
        \multicolumn{17}{c}{}
        \\
        \hline
        \multirow[c]{3}{*}{ Method } & \multirow[c]{3}{*}{ \shortstack{SfM \\ points}} & \multicolumn{15}{c}{Indoor Scene} \\
        \cline{3-17} & & \multicolumn{3}{c|}{ room } & \multicolumn{3}{c|}{ counter } & \multicolumn{3}{c|}{ kitchen} & \multicolumn{3}{c|}{ bonsai } & \multicolumn{3}{c}{ average } \\
        
        & & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$  \\
        \hline

        
        3DGS & cluster  & 29.980& 0.899& 0.256& 27.561& 0.878& 0.242& 30.132& 0.915&0.142& 31.004& 0.927& 0.227& 26.415& 0.780& 0.258\\

        3DGS & <10\%  & \second {30.795} & 0.908& 0.243& \third 28.523& \third 0.896& 0.223& 30.120& 0.915&0.140& 31.625& 0.934& 0.221& 26.893& 0.793& 0.247\\

        3DGS  & full  & \third 30.632&  \best{0.914}&  \best{0.220}&  \second{28.700}& \best{ 0.905}&  \best{0.204}&  \third 30.317&  \best{0.922}&  \best{0.129}&  \best{31.980}&  \best{0.938}&  \best{0.205}& \second{27.205} &  \best{0.815} & \best{0.214}  \\
        \hline

        Ours & cluster  & 30.546& \third 0.909& \third 0.239& 28.098& 0.892& \third 0.218& \second{31.361}& \best{0.922}& \third 0.134& \third 31.638& \third \third 0.935& \third 0.217& \third 27.188& \third 0.810& \third 0.222\\

        Ours & <10\% & \best{30.843}& \second{0.912} & \second{0.230} & \best{28.703} & \second{0.902} & \second{0.209} &\best{31.364}& \best{0.922}& \second{0.133} &  \second{31.829}& \best{0.938}& \second{0.214}&  \best{27.384}& \best{0.815}& \second{0.217}\\

        \hline
    \end{tabular}}

    \label{tab:sparse_mip360}
\end{table*}


==> supple_assets/table/SfMnoise_table.tex <==
\begin {table*}[t]
    \caption{\textbf{Quantitative comparison on Mip-NeRF360 dataset with various initilize methods}. We compare our method with the DSV random initialization method described in the original 3DGS~\cite{kerbl20233d} and noise SfM method. We report PSNR, SSIM, LPIPS and color each cell. }
    \vspace{-5pt}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
        \Xhline{3\arrayrulewidth}
        \multicolumn{16}{c}{Outdoor Scene} \\
        \hline \multirow[b]{2}{*}{ Method } & \multicolumn{3}{c|}{ bicycle } & \multicolumn{3}{c|}{ flowers } & \multicolumn{3}{c|}{ garden } & \multicolumn{3}{c|}{ stump } & \multicolumn{3}{c}{ treehill }\\
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ &PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$  \\
        \hline
        
        3DGS (DSV)  & - & - & - &  - & - & - &  - & - & - &  - & - & - &  - & - & -  \\

        3DGS (Noise)  & - & - & - &  - & - & - &  - & - & - &  - & - & - &  - & - & -  \\

        \hlrow Ours (SLV) & - & - & - &  - & - & - &  - & - & - &  - & - & - &  - & - & -  \\

        \Xhline{3\arrayrulewidth}
        \multicolumn{16}{c}{}
        \\
        \Xhline{3\arrayrulewidth}
        \multicolumn{16}{c}{Indoor Scene} \\
        \hline & \multicolumn{3}{c|}{ room } & \multicolumn{3}{c|}{ counter } & \multicolumn{3}{c|}{ kitchen} & \multicolumn{3}{c|}{ bonsai } & \multicolumn{3}{c}{ average } \\
        
        Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$  \\
        \hline
    

        3DGS (DSV)  & - & - & - &  - & - & - &  - & - & - &  - & - & - &  - & - & -  \\

        3DGS (Noise)  & - & - & - &  - & - & - &  - & - & - &  - & - & - &  - & - & -  \\
        
        \hlrow Ours(SLV) & - & - & - &  - & - & - &  - & - & - &  - & - & - &  - & - & -  \\
        
        \Xhline{3\arrayrulewidth}
    \end{tabular}}

    \label{exp:supp_DLV}
    \vspace{-5pt}
\end{table*}




==> supple_assets/table/computation_table_memory.tex <==
\begin {table}[!hbt]
    \caption{\textbf{Memory size}\tablefootnote{Except for 3DGS(DSV) and Ours, we copied the memory size of different models from 3DGS~\cite{kerbl20233d}.}}
    \centering
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c|c|c|c}
        \toprule & Mip-NeRF360 &  Tanks\&Temples & Deep Blending \\
        \midrule 
        
        Plenoxels  & 2.1GB & 2.3GB & 2.7GB \\

        INGP-Base  & 13MB & 13MB & 13MB  \\

        INGP-Big & 48MB & 48MB & 48MB \\

        3DGS & 734MB & 411MB & 676MB \\

        3DGS (DSV) & 592MB & 365MB & 582MB \\
        \hlrow Ours & 581MB & 359MB & 545MB \\

    \end{tabular}
    }

    \label{exp:memory_size}
\end{table}

==> supple_assets/table/movement.tex <==
\begin {table}[!hbt]
    \caption{\textbf{Analysis of points movement}}
    \centering
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{l|c|c|c}
        \toprule  & 3DGS (SfM) & 3DGS (Random) & Ours (Random) \\
        \midrule
        
        Means  & 0.349 &  0.184& 12.100\\

        Stds of movement & 0.726& 0.297& 18.600\\

        Top 1\% & 3.418& 1.524& 82.721\\
        Top 5\% & 1.444& 0.714& 35.486\\
        Top 10\% & 0.898& 0.458& 24.866\\
        \bottomrule
    \end{tabular}
    }

    \label{tab:movement}
\end{table}



